A First Look into DeFi Oracles

Recently emerging Decentralized Finance (DeFi) takes the promise of cryptocurrencies a step further, leveraging their decentralized networks to transform traditional financial products into trustless and transparent protocols that run without intermediaries. However, these protocols often require critical external information, like currency or commodity exchange rates, and in this respect they rely on special oracle nodes. In this paper, we present the first study of DeFi oracles deployed in practice. First, we investigate designs of mainstream DeFi platforms that rely on data from oracles. We find that these designs, surprisingly, position oracles as trusted parties with no or low accountability. Then, we present results of large-scale measurements of deployed oracles. We find and report that prices reported by oracles regularly deviate from current exchange rates, oracles are not free from operational issues, and their reports include anomalies. Finally, we compare the oracle designs and propose potential improvements.

==> algo/accountability.tex <==
\begin{algorithm}[!h]
    \caption{Accountability Contract.}
    \label{alg:accountablecontract}
    \SetAlgoVlined
    $mapping(address \Rightarrow \textlangle manifest,~deposit\textrangle)~Oracles$\\
    $struct~report\{unit~timestamp,~float~deviation\}$\\
    \medskip
    \SetKwProg{func}{function}{}{}
    \func{deposit(manifestAddr)}{
        Oracles[msg.sender].manifest $\leftarrow$ manifestAddr;\\
        Oracles[msg.sender].deposit $\mathrel{{+}{=}}$ msg.value;
    }
    
    \func{punish(oracle, report)}{
        \If{!checkMisbehavior(oracle, report)}
        {	
        	msg.sender.transfer(Oracles[oracle].deposit) \\
        	Oracles[oracle].deposit $\leftarrow$ 0
        }
    }
    
    \func{checkMisbehavior(oracle, report)}{
    	\texttt{/*~check late or missing reports~*/}\\
        \If{report.timestamp is late or report is NULL}
        {\Return~~{\it False}}
    	\texttt{/*~check high deviation~*/}\\
		\If{report.deviation $\geq$ Oracles[oracle].manifest.get().precision}
        {\Return~~{\it False}}
        \Return~~{\it True}
    }
    
\end{algorithm}

==> algo/manifest.tex <==
\begin{algorithm}[!h]
    \caption{Manifest Contract.}
    \label{alg:manifestcontract}
    \SetAlgoVlined
    $address~owner,~string[]~sources$\\
    $unit256~frequency,~float~precision$\\
    \medskip
    \texttt{/*~{\it sources}: the claimed data sources~*/}\\
	\texttt{/*~{\it frequency}: intended frequency of updates~*/}\\
	\texttt{/*~{\it precision}: maximum tolerated deviation~*/}\\
    \SetKwProg{func}{function}{}{}
    \func{constructor(src, freq, prec)}{
        owner $\leftarrow$ msg.sender, sources $\leftarrow$ src\\
        frequency $\leftarrow$ freq, precision $\leftarrow$ prec\\
    }

    \func{set(src, freq, prec)}{
        assert(owner == msg.sender), sources $\leftarrow$ src\\ 
        frequency $\leftarrow$ freq, precision $\leftarrow$ prec\\ 
    }
    
    \func{get()}{
        \Return (sources, frequency, precision)
    }
\end{algorithm}


==> fig/ampleforth-code.tex <==
\begin{figure}[th!]
% \setlength{\belowcaptionskip}{-0.8cm}
% \setlength{\algomargin}{5em}
% \lstset{numbers=left,xleftmargin=2em,frame=single,framexleftmargin=1.5em}
\lstset{numbers=left,xleftmargin=2em}


	\begin{lstlisting}[language=Solidity]
contract MedianOralce{
	function getReportData()
        returns (uint256, bool)
    {
        uint256 minValidTimestamp =  now.sub(reportExpirationTimeSec);
        uint256 maxValidTimestamp =  now.sub(reportDelaySec);
        for (uint256 i = 0; i < reportsCount; i++) {
            ......
            uint256 reportTimestampRecent = reports[index_recent].timestamp;
            if (reportTimestampRecent > maxValidTimestamp) {
                // Recent report is too recent.
                uint256 reportTimestampPast = providerReports[providerAddress][index_past].timestamp;
                if (reportTimestampPast < minValidTimestamp) {
                    // Past report is too old.
                    emit ReportTimestampOutOfRange(providerAddress);
                } else if (reportTimestampPast > maxValidTimestamp) {
                    // Past report is too recent.
                    emit ReportTimestampOutOfRange(providerAddress);
                } else {
                    // Using past report.
                    validReports[size++] = providerReports[providerAddress][index_past].payload;
                }
            } else {
                // Recent report is not too recent.
                if (reportTimestampRecent < minValidTimestamp) {
                    // Recent report is too old.
                    emit ReportTimestampOutOfRange(providerAddress);
                } else {
                    // Using recent report.
                    validReports[size++] = providerReports[providerAddress][index_recent].payload;
                }
            }
        }
        if (size < minimumProviders) {
            return (0, false);
        }
        return (computeMedian(validReports, size), true);
    }
	
}


	\end{lstlisting}
\caption{The \texttt{getReportData} method of \texttt{MedianOracle} contract of AmpleForth.}
\label{fig:getreportdata}
\end{figure}

==> fig/compound-code.tex <==
\begin{figure}[th!]
% \setlength{\belowcaptionskip}{-0.8cm}
% \setlength{\algomargin}{5em}
% \lstset{numbers=left,xleftmargin=2em,frame=single,framexleftmargin=1.5em}
\lstset{numbers=left,xleftmargin=2em}


	\begin{lstlisting}[language=Solidity]
contract OpenOralce{
	function postPrices(bytes[] calldata messages, bytes[] calldata signatures, string[] calldata symbols) external {
        require(messages.length == signatures.length, "messages and signatures must be 1:1");
        // Save the prices
        for (uint i = 0; i < messages.length; i++) {
            OpenOraclePriceData(address(data)).put(messages[i], signatures[i]);
        }
        // Try to update the median
        for (uint i = 0; i < symbols.length; i++) {
            string memory symbol = symbols[i];
            uint64 medianPrice = medianPrice(symbol, sources);
            uint64 anchorPrice = OpenOraclePriceData(address(data)).getPrice(anchor, symbol);
            if (anchorPrice == 0) {
                emit PriceGuarded(symbol, medianPrice, anchorPrice);
            } else {
                uint256 anchorRatioMantissa = uint256(medianPrice) * 100e16 / anchorPrice;
                // Only update the view's price if the median of the sources is within a bound, and it is a new median
                if (anchorRatioMantissa <= upperBoundAnchorRatio && anchorRatioMantissa >= lowerBoundAnchorRatio) {
                    // only update and emit event if the median price is new, otherwise do nothing
                    if (prices[symbol] != medianPrice) {
                        prices[symbol] = medianPrice;
                        emit PriceUpdated(symbol, medianPrice);
                    }
                } else {
                    emit PriceGuarded(symbol, medianPrice, anchorPrice);
                }
            }
        }
    }
}
	\end{lstlisting}
\caption{The \texttt{postPrices} method of \texttt{OpenOracle} contract of Compound.}
\label{fig:postrices}
\end{figure}

==> fig/deviation/ampleforth-deviation.tex <==
% \begin{subfigure}{.45\columnwidth}
%   \centering
%   \includegraphics[width=\textwidth]{fig/deviation/deviation-ampleforth.pdf}  
%   \caption{\af}
%   \label{fig:deviation-ampleforth-a}
% \end{subfigure}
\begin{subfigure}{.45\columnwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{fig/deviation/baseline-coinmarket-ampleforth.pdf}  
  \caption{Coinmarketcap}
  \label{fig:deviation-ampleforth-b}
\end{subfigure}
\begin{subfigure}{.45\columnwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{fig/deviation/baseline-bitfinex-ampleforth.pdf}  
  \caption{Bitfinex}
  \label{fig:deviation-ampleforth-c}
\end{subfigure}
\caption{Price deviations of the \af oracle from its price sources.}
\label{fig:deviation-ampleforth}


==> fig/deviation/compound-deviation.tex <==
% \begin{subfigure}{.45\columnwidth}
%   \centering
%   \includegraphics[width=\textwidth]{fig/deviation/deviation-compound.pdf}  
%   \caption{\cpd}
%   \label{fig:deviation-compound-a}
% \end{subfigure}
\begin{subfigure}{.45\columnwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{fig/deviation/baseline-coinbasepro-compound.pdf}  
  \caption{CoinbasePro}
  \label{fig:deviation-compound-b}
\end{subfigure}
\begin{subfigure}{.45\columnwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{fig/deviation/baseline-kraken-compound.pdf}  
  \caption{Kraken}
  \label{fig:deviation-compound-c}
\end{subfigure}
\caption{Price deviations of the \cpd oracle from its price sources.}
\label{fig:deviation-compound}


==> fig/deviation/maker-deviation.tex <==
% \begin{subfigure}{.23\textwidth}
%   \centering
%   \includegraphics[width=1.0\linewidth]{fig/deviation/deviation-makerdao.pdf}  
%   \caption{\maker}
%   \label{fig:deviation-makerdao-a}
% \end{subfigure}
\begin{subfigure}{.45\columnwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{fig/deviation/baseline-coinmarket-maker.pdf}  
  \caption{Coinmarketcap}
  \label{fig:deviation-makerdao-b}
\end{subfigure}
\begin{subfigure}{.45\columnwidth}
  \centering
  \includegraphics[width=0.9\textwidth]{fig/deviation/baseline-bitfinex-maker.pdf}  
  \caption{Bitfinex}
  \label{fig:deviation-makerdao-b}
\end{subfigure}
\caption{Price deviations of the \maker oracle from its price sources.}
\label{fig:deviation-makerdao}


==> fig/deviation/multiple-deviation.tex <==
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{fig/deviation/multiple-synthetix.pdf}  
  \caption{\synt}
  \label{fig:multiple-deviation-a}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{fig/deviation/multiple-makerdao.pdf}  
  \caption{\maker}
  \label{fig:multiple-deviation-b}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{fig/deviation/multiple-compound.pdf}  
  \caption{\cpd}
  \label{fig:multiple-deviation-c}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{fig/deviation/multiple-ampleforth.pdf}  
  \caption{\af}
  \label{fig:multiple-deviation-d}
\end{subfigure}
\caption{Deviation comparison (per platform) among different sources.} 
\label{fig:multiple-deviation}


==> fig/deviation/synthetix-deviation.tex <==
% \begin{subfigure}{.24\textwidth}
%   \centering
%   \includegraphics[width=.8\linewidth]{fig/deviation/deviation-synthetix.pdf}  
%   \caption{\synt}
%   \label{fig:deviation-synthetix-a}
% \end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{fig/deviation/baseline-coinmarket-synthetix.pdf}  
  \caption{Coinmarketcap}
  \label{fig:deviation-synthetix-b}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{fig/deviation/baseline-bitfinex-synthetix.pdf}  
  \caption{Bitfinex}
  \label{fig:deviation-synthetix-c}
\end{subfigure}
\begin{subfigure}{.24\textwidth}
  \centering
  \includegraphics[width=0.9\linewidth]{fig/deviation/baseline-bittrex-synthetix.pdf}  
  \caption{Bittrex}
  \label{fig:deviation-synthetix-d}
\end{subfigure}
\caption{Price deviations of the \synt oracle from its price sources.}
\label{fig:deviation-synthetix}


==> fig/market-price/market-price.tex <==
\begin{subfigure}{0.24\textwidth}
  \centering
  \includegraphics[width=0.3\textwidth]{fig/market-price/market-makerdao.pdf}  
  \caption{SAI}
  \label{fig:market-price-a}
\end{subfigure}
\begin{subfigure}{0.24\textwidth}
  \centering
  \includegraphics[width=0.3\textwidth]{fig/market-price/market-ampleforth.pdf}  
  \caption{AMPL}
  \label{fig:market-price-b}
\end{subfigure}
\begin{subfigure}{0.24\textwidth}
  \centering
  \includegraphics[width=0.3\textwidth]{fig/market-price/market-synthetix.pdf}  
  \caption{SNX}
  \label{fig:market-price-c}
\end{subfigure}
\caption{Historical prices of selected DeFi assets.}
\label{fig:market-price}     


==> fig/price-volatility.tex <==
% \begin{wrapfigure}[8]{r}{0.8\textwidth}
\begin{figure}[!h]
% \vspace{-0.8cm}
\centering
\includegraphics[width=1.0\linewidth]{fig/market-price/market-price.pdf}
\caption{Historical prices of selected DeFi assets.}
\label{fig:market-price}     
% \end{wrapfigure}
\end{figure}
